Interference Mitigation and Resource Allocation in Underlay Cognitive Radio Networks

Due to ever increasing usage of wireless devices and data hungry applications, it has become necessary to improve the spectral efficiency of existing wireless networks. One way of improving spectral efficiency is to share the spectrum amongst different coexisting networks and serve multiple devices simultaneously. Spectrum sharing mechanisms for coexistence of a licensed network, such as LTE, with an unlicensed network, such as Wi-Fi, are being considered in the recent literature and standardizations. In order to enable the coexistence between licensed and unlicensed users, it is necessary to include interference mitigation techniques to protect the licensed primary users (PUs) from harmful interference. Typical interference mitigation mechanisms are based on spectrum sensing and cognitive radio (CR), wherein unlicensed secondary users (SUs) observe the spectrum and utilize it when licensed PUs are inactive. Thus, the SUs utilize empty time-slots in the shared spectrum to avoid the interference. The spectral efficiency can be further improved if the SUs are allowed to transmit concurrently with PUs by exploiting the spatial dimension provided by multiple antenna techniques. The underlay CR paradigm allows such coexistence where SUs transmit its signal in the same time-slots as PUs by exploiting the spatial and frequency resources in the network. In order to exploit the spatial dimension, SUs can utilize the location coordinates of PUs to steer its signal away from PUs to mitigate the interference. The SU transmitter can also employ multiple antenna techniques to serve a large number of devices. Further, the SUs can utilize frequency bands occupied by PUs by dynamically selecting the frequency band that provides the highest rate. In this work, we develop techniques for PU location estimation, spatial resource allocation and frequency band selection for SUs in underlay CR networks.

==> include/introduction.tex <==

%
% introduction.tex
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>.
% $Id: demo2int.tex,v 1.1 1996/01/12 18:13:58 johnh Exp $
%

\chapter{Introduction}

\noindenthack
Filing services are one of the most user-visible
  parts of the operating system,
  so it is not surprising that 
  many new services are proposed
  by researchers
  and that a variety of third parties are interested in providing
  these solutions.
Of the many innovations which have been proposed,
  very few have become widely available
  in a timely fashion.
We believe this delay results from two deficiencies
  in practices of current file-system development.
First,
  file systems are large and difficult to implement.
This problem is compounded because
  no good mechanism exists to allow
  new services to build on those which already exist.
Second,
  file systems today are built around a few fixed interfaces
  which fail to accommodate the change and evolution inherent in
  operating systems development.
Today's filing interfaces vary from
  system to system,
  and even between point releases of a 
  single operating system.
These differences greatly complicate and therefore discourage
  third-party development and adoption of filing extensions.

These problems raise barriers to the widespread
  development, deployment, and maintenance of new filing
  services.
The thesis of this dissertation is that
  a layered,
  \emph{stackable} structure
  with an \emph{extensible} interface
  provides a much better methodology
  for file-system development.
We propose construction of filing services from a number
  of potentially independently developed modules.
By stackable,
  we mean that these modules are bounded by
  identical, or \emph{symmetric}, interfaces above and below.
By extensible, we mean that these interfaces
  can be independently changed by multiple parties,
  without invalidating existing or future work.

To validate this thesis we developed a
  framework supporting stackable file-systems
  and used that framework to construct several
  different filing services.
This dissertation describes the design,
  implementation,
  and evaluation of this system.


% \input{motivation}



% \section{Related Work}
%	\label{sec:intro_related_work}

% ...


% LocalWords:  Posix Novell's Netware Kernighan Madnick Alsop NeFS PostScript
% LocalWords:  Rosenthal SunSoft NEEDSWORK Wong


==> include/macros.tex <==

%
% thesis_macros
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>
%

% \RequirePackage{johnh_general}

\RequirePackage{ifthen}

% \def\epsfreduction{0.667}
\def\epsfgraphreduction{0.9}

\newcommand\comment[1]{{[\sffamily #1]}}

%
% TeX seems to want to indent after chapters,
% although it shouldn't.  Rather than argue
% with it, I work around it manually by putting this
% hack in the right places:
\newcommand{\noindenthack}{\noindent}


\newcommand{\fwling}{featherweight layering}
\newcommand{\fwls}{featherweight layers}
\newcommand{\fwl}{featherweight layer}

\newcommand{\Fwling}{Featherweight layering}
\newcommand{\Fwls}{Featherweight layers}
\newcommand{\Fwl}{Featherweight layer}

\newcommand{\FwLing}{Featherweight Layering}
\newcommand{\FwLs}{Featherweight Layers}
\newcommand{\FwL}{Featherweight Layer}

\newcommand{\xvop}[2]{{\scomputer {{#1}\_{#2}}}}
\newcommand{\vop}[1]{\xvop{vop}{#1}}

\newcommand{\usec}{$\mu$seconds}
\newcommand{\unix}{Unix}

\newcommand{\dotdot}{\scomputer{..}}

\newenvironment{mycode}%
	{\small
	}{%
	}

\newcommand{\mylangle}{\langle}
\newcommand{\myrangle}{\rangle}
\newcommand{\myrightarrow}{\rightarrow}


%
% Sizes of various things:
%
  \newcommand{\tablesize}{\normalsize}
  \newcommand{\computertablesize}{\small}
  \newcommand{\bibliographysize}{\normalsize}

  %
  % Another space-saver:  shrink the figures and graphs.
  %
 \def\epsfreduction{0.85}
 \def\epsfgraphreduction{0.9}   % should be left at 0.9 with two-column text
% \def\epsfsize#1#2{\epsfreduction#1}

%\newcommand{\appendixnumbering}{
%	\renewcommand{\thechapter}{\Alph{chapter}}
%	\setcounter{chapter}{0}
%	}

\newenvironment{functions}%
	{\begin{description}}%
	{\end{description}}

\makeatletter
  \newcommand{\SubmitSingleSpace}{
    \ifissubmit
      \renewcommand\baselinestretch{\@singlespacing}\@normalsize
    \fi
  }
  \newcommand{\SubmitDoubleSpace}{
    \ifissubmit
      \renewcommand\baselinestretch{\@doublespacing}\@normalsize
    \fi
  }
\makeatother


\iffalse
Figure drawing style guide:

layer labels:
	helvetica 12pt bold
	(short acronyms) helvetica 14pt bold

spacing:  8 pixels
each layers will be 3 high and 7 or 7.5 wide

or spacing: 8 pts
each layer will be 4 high and 10 wide

boxes and vnode links are line #2
\fi



==> include/main.tex <==

%
% main.tex
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>.
% $Id: demo2big.tex,v 1.2 1996/01/16 18:57:04 johnh Exp $
%

\input{include/macros}

\begin{document}

\input{include/titlepages}
\input{include/introduction}
%...
%\input{stacking_model}
%\input{stacking_techniques}
%\input{stacking_implementation}
%\input{stacking_evaluation}
%\input{coherence_architecture}
%\input{coherence_implementation}
%\input{coherence_evaluation}
%\input{fwl_implementation}
%\input{fwl_evaluation}
%\input{related_work}
%\input{conclusion}

%\appendix
%\input{stacking_appendix}
%\input{coherence_appendix}

%\bibliographystyle{uclathes}
%\bibliography{ficus,thesis}

%\input{colophon}

\end{document}



==> include/titlepages.tex <==

%
% Title pages of the thing
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>.
%



\title{Stackable Design of File Systems}
\author{John~Shelby Heidemann}


\department{Computer Science}
\degreemonth{September}
\degreeyear{1995}

\chair{Gerald~J.~Popek}
\chair{D.~Stott Parker}
\member{Richard~Muntz}
\member{Rajive~L.~Bagrodia}
\member{Kirby~A.~Baker}

\dedication{\textsl{Are you dedicated?}}

\acknowledgments{
Ack!  P'tui.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% vita
%
\vitaitem{1968}{B.S., Computer Science, Caribou University}
\vitaitem{etc.}{etc.}
\vitaitem{1995}{Graduated, UCLA}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% publications
%

\publication{
	Richard~G.\ Guy, John~S.\ Heidemann, Wai Mak, Thomas~W.\ Page,~Jr.,\ 
	  Gerald~J.\ Popek, and Dieter Rothmeier.
	Implementation of the Ficus
	  replicated file system.
	In \emph{USENIX Conference Proceedings}, pages
	  63--71.
	USENIX, June 1990.
}

\publication{
	etc.
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\include{abstract}

%
% I built a custom title page to do what I want.  So sue me.
% NEEDSWORK:  I had to copy some stuff from uclathti.sty.
%
\makeatletter
  \newcommand{\CustomTitlePage}{
    \begin{titlepage}
      \ColumnSave
      \vspace*{1.5in}   % a hacky way to center.  TeX didn't like \vfill.
      \begin{center}
  
      {\bfseries\huge \@title} \\
      \vskip 48pt plus0pt minus18pt
  
      {\large \@author} \\
      \vskip 12pt plus0pt minus3pt
      {\large University of California, Los Angeles} \\
      \vskip 6pt plus0pt minus2pt
      {\large \@degreemonth, \@degreeyear} \\
      \vskip 48pt plus0pt minus18pt
  
      \normalsize A \@thesisname\
      submitted in partial satisfaction \\
      of the requirements for the degree \\
      \@degreename\if@department\ in \@department \fi\\
      \vskip 24pt plus0pt minus6pt

      \normalsize
	UCLA Computer Science Department \\
	Technical Report UCLA-CSD-950032 \\
      \vskip 24pt plus0pt minus6pt

      \textbf{Thesis committee:} \\
      \ifnum\c@chairs<1
        \typeout{No committee chair.}
      \else\ifnum\c@chairs<2
        \@chairA, chair \\
      \else\ifnum\c@chairs<3
        \@chairA, co-chair \\
        \@chairB, co-chair \\
      \else\ifnum\c@chairs<4
        \@chairA, co-chair \\
        \@chairB, co-chair \\
        \@chairC, co-chair \\
      \fi\fi\fi\fi
      \ifnum\c@members<1 \typeout{No non-chair committee members.}\fi
      \ifnum\c@members>0 \@memberA \\ \fi
      \ifnum\c@members>1 \@memberB \\ \fi
      \ifnum\c@members>2 \@memberC \\ \fi
      \ifnum\c@members>3 \@memberD \\ \fi
      \ifnum\c@members>4 \@memberE \\ \fi
      \ifnum\c@members>5 \@memberF \\ \fi

      \end{center}
    \end{titlepage}
  }

  \newcommand{\CustomAcknowledgePage}{
  \chapter*{Acknowledgments}

  \@acknowledgments
  }
\makeatother

\ifissubmit
  \makeintropages
\else
  \makeatletter
    \pagenumbering{roman}
    \CustomTitlePage
    \@makecopyrightpage
    \@makededication
    \tableofcontents
    \listoffigures
    \listoftables
    \cleardoublepage
    \@makeabstractpage{1.0}
    \CustomAcknowledgePage
%    \@makevitapage

    \cleardoublepage
    \pagestyle{headings}
    \pagenumbering{arabic}
    \setcounter{page}{1}
  \makeatother
\fi


% LocalWords:  Stott Muntz Ted Yu Wu Michial Gunter Stovall Salomone Louie Qian
% LocalWords:  Qin Weidner McKusick Pendry Minshall kitrace Ousterhout CSD ftp
% LocalWords:  Administrativia csd ps HyperCard Yarvis Alexy Rudenko pt Los co
% LocalWords:  degreemonth degreeyear thesisname degreename chairA chairB roman
% LocalWords:  chairC memberA memberB memberC memberD memberE memberF arabic
% LocalWords:  makecopyrightpage makededication makeabstractpage Monique http
% LocalWords:  Bennarosh www html

